A multiple attribute model resolves a conflict between additive and multiplicative models of incentive salience

A model of incentive salience as a function of stimulus value and interoceptive state has been previously proposed. In that model, the function differs depending on whether the stimulus is appetitive or aversive; it is multiplicative for appetitive stimuli and additive for aversive stimuli. The authors argued it was necessary to capture data on how extreme changes in salt appetite could move evaluation of an extreme salt solution from negative to positive. We demonstrate that arbitrarily varying this function is unnecessary, and that a multiplicative function is sufficient if one assumes the incentive salience function for an incentive (such as salt) is comprised of multiple stimulus features and multiple interoceptive signals. We show that it is also unnecessary considering the dual-structure approach-aversive nature of the reward system, which results in separate weighting of appetitive and aversive stimulus features.

==> document-sections/04further-notes.tex <==

\subsection{Alternative approaches to approach and avoidance}

\subsubsection{By `expectancy'}
If we assume separate positive/negative expectancies for each mode (still assuming a constant loss aversion across modes)...
\begin{align}\label{eq:SaltSugarModelTindellExpectancy}
\tilde r(\mvector{r},\mvector{\kappa}) = & (e_{\text{Na},p}-\lambda e_{\text{Na},n})\kappa_{\text{Na}} r_{\text{Na}} \\  \nonumber
& + (e_{h,p}-\lambda e_{h,n})\kappa_{h} r_{h} \\ \nonumber
& + (e_{\text{Glc},p}-\lambda e_{\text{Glc},n})\kappa_{\text{Glc}} r_{\text{Glc}} \nonumber
\end{align}

...or if we assume constant positive/negative expectancy (is this practical? I don't think so)

\begin{equation}\label{eq:SaltSugarModelTindellConstantExpectancy}
\tilde r(\mvector{r},\mvector{\kappa})=(e_p-\lambda e_n)(\kappa_{\text{Na}} r_{\text{Na}}+\kappa_{h} r_{h} + \kappa_{\text{Glc}} r_{\text{Glc}})
\end{equation}


\subsection{Alternative model}

One thing to do with rats is to make food obnoxious by putting quinine in it. If we do a version with a salt and quinine solution, we'd find that a non-deprived rat is going to really avoid the solution, but as soon as they are salt-deprived, they'll go for it because salt desire will override aversion to the quinine. The point being: maybe `tastiness' is an intrinsic term to add to the model.





\subsubsection{Inspiration from the OpAL model}

Could we use the OpAL model to build in positive and negative expectancies? I don't think there's much to learn directly from the OpAL model.



\section{Further modeling}

I am still working on extending this further to demonstrate how the model is related to \cite{keramati2014homeostatic}, how modeling approach and avoid separately can be useful for modeling behavior \cite{READ2017237}, and how we can extend the model to break up the $1:1$ relationship between each of the items in this model.



==> preamble.tex <==
\usepackage[american]{babel}

\usepackage[backend=biber,style=apa]{biblatex}

\input{latex_customization/math_customization}
\input{latex_customization/general_customization.tex}


\DeclareLanguageMapping{american}{american-apa}
\addbibresource{biblio.bib}


\usepackage{amsmath}
